Quadratic Tangles in Planar Algebras

In planar algebras, we show how to project certain simple "quadratic" tangles onto the linear space spanned by "linear" and "constant" tangles. We obtain some corollaries about the principal graphs and annular structure of subfactors.

==> FIGURES/4box <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 1200 7200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 1200 1200 6000 1200 7200 600
4 0 0 50 0 0 24 0.0000 4 180 180 3000 1275 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4725 1275 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 5925 1275 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 7125 675 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 7125 1875 o\001
4 0 0 50 0 0 32 0.0000 4 195 255 1050 1420 *\001


==> FIGURES/combinatorial <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 1200 2400 3000 2400 4200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2400 4125 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2400 9000 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 1650 7500 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8325 1650 8325 2400
4 0 0 50 0 0 30 0.0000 4 195 255 1050 2625 *\001
4 0 0 50 0 0 30 0.0000 4 195 255 5250 2625 *\001
4 0 0 50 0 0 24 0.0000 4 180 7470 1650 2475 o    o      o                              o     o         o       o      o\001
4 0 0 50 0 0 24 0.0000 4 180 180 3525 2100 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4125 1650 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 3525 2925 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4050 3375 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 7425 1800 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 8250 1800 o\001


==> FIGURES/comult <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 2507.661 1480.645 2700 975 2100 1125 2025 1725
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3571.323 3765.441 3750 4575 4350 4050 4200 3225
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 3262 3075 2694 2694 675 2325 5850 3825
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 3187 3937 857 857 2400 3600 3975 4275
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 3112 1687 803 803 2475 1200 3750 2175
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 3225 3600 2325
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3000 900 3225 375
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3375 900 3600 375
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 3750 2175 4575 3225 4125 5625
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3600 1050 3975 450
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 2700 4650 2325 5625
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3075 4800 2850 5775
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3000 3075 2700 2400
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3300 3075 3150 2475
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 3525 4725 3450 5775
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 2
	 2025 1725 2775 3150
	 0.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 2625 3300 1575 2025 2025 675
	 0.000 -1.000 0.000
4 0 0 50 0 0 24 0.0000 4 135 180 2100 4200 *\001
4 0 0 50 0 0 24 0.0000 4 135 180 2175 1725 *\001
4 0 0 50 0 0 24 0.0000 4 135 180 1275 1575 *\001
4 0 0 50 0 0 24 0.0000 4 255 240 3000 4125 R\001
4 0 0 50 0 0 24 0.0000 4 330 270 2925 1800 Q\001


==> FIGURES/haagerup <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 1200 2400 3000 2400 4200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2400 9000 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 1650 7500 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8325 1650 8325 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 1500 4650 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4125 3300 4425 3525
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2400 4125 3300
4 0 0 50 0 0 30 0.0000 4 165 210 1050 2625 *\001
4 0 0 50 0 0 30 0.0000 4 165 210 5250 2625 *\001
4 0 0 50 0 0 24 0.0000 4 180 7470 1650 2475 o    o      o                              o     o         o       o      o\001
4 0 0 50 0 0 24 0.0000 4 180 180 3525 2100 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4125 1650 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4050 3375 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 7425 1800 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 8250 1800 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 3525 2925 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4575 1350 o\001
4 0 0 50 0 0 24 0.0000 4 180 180 4425 3675 o\001


==> FIGURES/pg1 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 600 1200 75 75 600 1200 675 1200
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1800 1200 75 75 1800 1200 1800 1275
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3000 1200 75 75 3000 1200 3000 1275
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5400 1200 75 75 5400 1200 5475 1200
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5400 300 75 75 5400 300 5400 375
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 1200 75 75 6600 1200 6675 1200
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 300 75 75 6600 300 6600 375
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 7800 1200 75 75 7800 1200 7875 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 675 1200 1725 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 1200 2925 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3075 1200 3450 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1200 5325 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 1125 5400 375
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 1125 6600 375
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5475 1200 6525 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6675 1200 7725 1200
4 0 0 50 0 0 25 0.0000 4 30 1440 3600 1200 .  .  .  .  .  .\001


==> FIGURES/pg2 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 600 1200 75 75 600 1200 675 1200
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1800 1200 75 75 1800 1200 1800 1275
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3000 1200 75 75 3000 1200 3000 1275
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5400 1200 75 75 5400 1200 5475 1200
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 825 75 75 6600 825 6600 900
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 7800 450 75 75 7800 450 7800 525
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 1575 75 75 6600 1575 6675 1575
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 7800 1875 75 75 7800 1875 7875 1875
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 675 1200 1725 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 1200 2925 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3075 1200 3450 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1200 5325 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6675 1575 7725 1875
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5475 1200 6525 1510
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6675 815 7725 450
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5475 1200 6525 838
4 0 0 50 0 0 25 0.0000 4 30 1440 3600 1200 .  .  .  .  .  .\001

